Bridging Critical Gaps in Convergent Learning: How Representational Alignment Evolves Across Layers, Training, and Distribution Shifts

Understanding convergent learning -- the degree to which independently trained neural systems -- whether multiple artificial networks or brains and models -- arrive at similar internal representations -- is crucial for both neuroscience and AI. Yet, the literature remains narrow in scope -- typically examining just a handful of models with one dataset, relying on one alignment metric, and evaluating networks at a single post-training checkpoint. We present a large-scale audit of convergent learning, spanning dozens of vision models and thousands of layer-pair comparisons, to close these long-standing gaps. First, we pit three alignment families against one another -- linear regression (affine-invariant), orthogonal Procrustes (rotation-/reflection-invariant), and permutation/soft-matching (unit-order-invariant). We find that orthogonal transformations align representations nearly as effectively as more flexible linear ones, and although permutation scores are lower, they significantly exceed chance, indicating a privileged representational basis. Tracking convergence throughout training further shows that nearly all eventual alignment crystallizes within the first epoch -- well before accuracy plateaus -- indicating it is largely driven by shared input statistics and architectural biases, not by the final task solution. Finally, when models are challenged with a battery of out-of-distribution images, early layers remain tightly aligned, whereas deeper layers diverge in proportion to the distribution shift. These findings fill critical gaps in our understanding of representational convergence, with implications for neuroscience and AI.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} 
    \item[] Justification: Yes, we have described these in the discussion section.
    
\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} 
    \item[] Justification: No theoretical results are discussed in this paper.
    
    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} 
    \item[] Justification: Yes, we discuss our experimental setup in both Section 3 and Appendix A1.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} 
    \item[] Justification: All datasets are publicly available. We provide a link to our code in the Supplementary section.
    
\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, we describe these details in Appendix A1.
    
\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} 
    \item[] Justification: Yes, they are displayed in all figures.
    
\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} 
    \item[] Justification: Yes, all models and subsequent analyses were performed on an NVIDIA A40 GPU. Training an ImageNet model took $\approx 80$ hours and CIFAR100 models took $\approx 4$ hours. 
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} 

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} 
    \item[] Justification: We don't foresee any negative societal impact of our work.
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} 
    \item[] Justification: In our knowledge, we don't use any model that may pose a risk for misuse.
    
\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} 
    \item[] Justification: Yes (\emph{e.g.,}~\cite{deng2009imagenet},~\cite{geirhos2018imagenet})

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No new assets are introduced in this paper.
    
\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    
\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} 
    
\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} 
    \item[] Justification: We didn't use LLMs to conduct any original scientific work or hypotheses.
    
\end{enumerate}



==> figures-code/inter-model-sm.tex <==
\begin{figure}[htbp!]
    \centering
    % cifar100
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_resnet50_soft_match_cifar100_comparison.png}\hfill
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg16_soft_match_cifar100_comparison.png}\hfill
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg19_soft_match_cifar100_comparison.png}\hfill 
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/vgg16_resnet50_soft_match_cifar100_comparison.png}\hfill
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/vgg19_resnet50_soft_match_cifar100_comparison.png}\hfill 
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/vgg16_vgg19_soft_match_cifar100_comparison.png}\\
    
    % imagenet
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_resnet50_soft_match_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg16_soft_match_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg19_soft_match_imagenet_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/resnet50_vgg16_soft_match_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet50_vgg19_soft_match_imagenet_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/vgg16_vgg19_soft_match_imagenet_comparison.png}
    \caption{\textbf{Inter-Model Soft-Match.} Identical to the preceding plot, we compute the layer-wise soft-matching score for all networks pairs ImageNet, similarly revealing consistent inter-layer relationships across architectures.}
    
    \label{tab:sm_inter_model} 
\end{figure}

==> figures-code/ood-amplification-swav.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{8pager/figures/nsd-results/self-supervised.png}
    \caption{Caption}
    \label{fig:ood-amplification-swav}
\end{figure}

==> figures-code/swav-hierarchy.tex <==
\begin{figure*}[htbp!]
    \centering
    \includegraphics[scale=0.5]{8pager/figures/network-hierarchy/r50_swav_imagenet.png}
    \caption{\textbf{Representational Convergence Across Network Hierarchy Using SwAV Training.} We evaluate representational alignment for a pair of SwAV-trained, ResNet50 backbone network on the ImageNet dataset. Error bars denote the standard deviation computed across 5-fold cross-validation.}
    \label{fig:swav-hierarchy}
\end{figure*}

==> yztwgkssnyyscymchgzppyswgzfcqwzw/acrossdistribution.tex <==
%\input{./figures-code/pearson-ood}
\subsection{Convergence across distribution shifts}
\label{sec:ood-results}
Having established alignment on in-distribution images, we next probed its robustness to distribution shift. We applied $17$ out-of-distribution (OOD) variants from ~\citep{geirhos2018imagenet} to ImageNet-trained CNNs. Dataset specifics are given in Appendix~\ref{sec: ood-dataset-details}.

% In the previous sections, we examined representational alignment under identical input training distributions. However, a critical question remains: does representational convergence persist under distribution shifts? To explore this, we analyzed the internal representations of ImageNet-trained DCNNs when exposed to OOD stimuli. We used $17$ OOD datasets from~\citep{geirhos2018imagenet}, all sharing the same $16$ coarse labels as ImageNet~\citep{deng2009imagenet}, allowing for a controlled comparison of representational alignment under varying distributional shifts. The specifics of each OOD dataset has been described in Sec.~\ref{sec: ood-dataset-details}.
%In the previous sections, we examined representational alignment under the same input distributions used for training. However, a critical question remains: does representational convergence persist under distribution shifts? To explore this, we analyzed the internal representations of ImageNet-trained DCNNs when exposed to OOD stimuli. We used $17$ OOD datasets from~\citep{geirhos2018imagenet}, all sharing the same $16$ coarse labels as ImageNet~\citep{deng2009imagenet}, allowing for a controlled comparison of representational alignment under varying distributional shifts. The specifics of each OOD dataset has been described in Sec.~\ref{sec: ood-dataset-details}.
\input{./figures-code/ood-amplification}
%\input{8pager/figures-code/pearson-ood}

% ood amplification
Using the Procrustes metric, we compute representational alignment on these datasets and observed a consistent pattern: OOD inputs amplify differences in the later layers of the networks, while early layers maintain comparable alignment levels between in-distribution and OOD stimuli (Fig.~\ref{fig:ood-amplification}). We hypothesize that this pattern arises because early layers capture universal features (\emph{e.g.,} edges, textures) that remain nearly identical across distributions, whereas later layers encode task-specific features that are sensitive to distributional shifts, thus amplifying the divergence between models.
%We computed representational alignment across these datasets using the Procrustes metric and observed a consistent pattern: OOD inputs amplify differences in the later layers of the networks, while early layers maintain comparable alignment levels between in-distribution and OOD stimuli (Fig.~\ref{fig:ood-amplification}). We hypothesize that this pattern arises as a result of early layers capturing basic, universal features (\emph{e.g.,} edges, corners, textures) that remain nearly identical across distributions, whereas later layers encode more task-specific features that are more sensitive to distributional shifts, thus amplifying the divergence between models.
We also found a strong correlation between representational alignment and OOD accuracy: datasets where models maintained higher accuracy show strong alignment and vice versa. This correlation is minimal in early layers, but progressively increases with network depth across all architectures (Fig.~\ref{fig: ood-convergence}); analogous trends appear in other networks Fig.~\ref{fig:ood-convergence-appendix}.
%Moreover, we found a strong correlation between representational alignment in later layers and the networks' classification accuracy on the OOD datasets. Datasets where models maintained higher accuracy showed stronger alignment, whereas datasets with lower accuracy exhibited weaker alignment. This correlation was notably weaker in early layers but increased progressively with network depth across all architectures (Fig.~\ref{fig: ood-convergence}). We extend these analyses to other vision networks in Fig.~\ref{fig:ood-convergence-appendix}.

These results have several important implications. First, early-layer alignment is remarkably stable---across random initializations and in-distribution and OOD inputs—indicating that these layers encode broadly transferable features that serve as a common scaffold for higher processing. Because this scaffold endures under distribution shift, one could plausibly improve OOD generalisation by fine-tuning only the later layers.  Second, these findings inform model-brain comparisons. Though diverse architectures and learning objectives yield similar brain predictivity~\citep{conwell2024large}, the amplified divergence of later-layer representations under OOD conditions suggests that OOD stimuli could be especially useful to distinguish and select between models whose representations closely mirror the brain.
\input{./figures-code/pearson-ood}
%These results have several important implications. First, the stability of early-layer alignment across distributions suggests that these layers encode generalizable features that are consistent across both network initializations and input distributions. This highlights their role as a shared foundation for higher-level processing, which becomes more specialized and sensitive to distribution shifts in later layers. Second, these findings inform model-brain comparisons. Prior studies have shown that diverse architectures and learning objectives can yield similar brain predictivity~\citep{conwell2024large}. However, the observed amplification of representational divergence in later layers under OOD conditions suggests that using OOD stimuli could be an effective strategy for distinguishing between models and identifying more brain-like models. 



==> yztwgkssnyyscymchgzppyswgzfcqwzw/acrosslayers.tex <==
\subsection{Evolution of Convergence Across the Network Hierarchy}
\label{sec: convergence-evolution}


%\input{./figures-code/privileged-axes-table}
\paragraph{How convergence varies with network depth.}
When comparing representational convergence across the network hierarchy for different seeds of the same architecture, we observe that convergence is strongest in the earliest layers and gradually diminishes in deeper layers (Fig.~\ref{fig:network-hierarchy}). This pattern is consistent across all three metrics and across networks trained on ImageNet. The high alignment in early layers likely arises because they capture fundamental, low-frequency features (\emph{e.g.,} edges, corners, contrast) that are universal across representations~\citep{rahaman2019spectral, bau2017network, zeiler2014visualizing}. In contrast, deeper layers, while still showing significant alignment $(> 0.5)$, exhibit greater variability due to their sensitivity to specific training conditions and noise. We also contrast this result with randomly initialized (untrained) networks as a baseline. We find that alignment scores across all metrics are consistently lower in untrained networks compared to their trained counterparts. This difference is especially pronounced in deeper layers: for instance, using the Procrustes metric, the mean alignment increases by $145.26\%$ in early layers (depth $<0.5$) and by $493.84\%$ in deeper layers (depth $>0.5$) following training. This trend also holds when comparing networks with different architectures, underscoring the robustness of hierarchical convergence across diverse models. Interestingly, a similar hierarchical trend is observed in human brain responses to visual stimuli (Appendix~\ref{sec: nsd-comparisons}).
\input{./figures-code/network-hierarchy}
% training evolution
%\input{./figures-code/inter-model-proc}
\input{./figures-code/inter-model-comparisons}
\paragraph{Minimal transformations needed to align representations.}
Across all layers, we find that alignment scores increase as the mapping functions become more permissive (\textcolor{mplgreen}{Permutation} $\rightarrow$ \textcolor{mplorange}{Procrustes} $\rightarrow$ \textcolor{mplblue}{Linear}), as expected. However, linear mappings provide only modest improvements over Procrustes correlations, indicating that rotational transformations are sufficient to capture the majority of alignment information. This suggests that the added flexibility of linear mappings---such as scaling and shearing---does not substantially enhance alignment beyond what is achieved with Procrustes transformations. Importantly, because Procrustes is symmetric, this result highlights that alignment reflects a deeper similarity in the geometric structure of representations, rather than merely the ability of one representation to predict another.



\paragraph{Simple permutations achieve significant alignment.}  
\label{par: privileged-axes}
Despite the strict constraints imposed by permutation-based alignment, Permutation scores achieve surprisingly high alignment levels, indicating a strong one-to-one correspondence between individual neurons across network instances---suggesting that convergent learning extends down to the single-neuron level, even without allowing for more flexible transformations.

\input{./figures-code/privileged-axes-table}

To further probe this result and assess the depth of convergent learning, we tested the sensitivity of permutation alignment to changes in the representational basis. 

Specifically, we applied a random rotation matrix $\bm{Q} \in \mathbb{R}^{n \times n}$ to the converged basis of a neural representation, where $n$ is the number of neurons in a given layer. The rotation matrix was sampled from a Haar distribution via a $QR$ decomposition, ensuring that all orthogonal matrices were equally likely. We then recomputed the Permutation score after applying this rotation.

We conducted this analysis by taking response matrices from two identical DCNNs (initialized with different random seeds) at a given convolutional layer, $\{\bm{X}_1, \bm{X}_2\} \in \mathbb{R}^{m \times n}$, where $m$ represents the number of stimuli. We applied the random rotation $\bm{Q}$ to one network’s responses and computed the resulting permutation-based correlation score, $s_{\text{perm}}(\bm{X}_1\bm{Q}, \bm{X}_2)$. This process was repeated across all convolutional layers, with the alignment differences summarized in Table~\ref{tab:perm-rotated}.


These rotations consistently reduced alignment, with a drop between $\sim 10-202\%$ for ResNet$18$ across all layers, for instance. This significant decrease highlights that the learned representations are \emph{not} rotationally invariant and the specific bases in which features are encoded is meaningfully preserved across networks. In other words, convergent learning aligns not just the overall representational structure but also the specific axes along which features are encoded. This observation echoes recent findings by~\citep{khosla2024privileged}, who report the existence of privileged axes in biological systems as well as the penultimate layer representations of trained artificial networks. %Interestingly, Vision Transformers (ViTs) exhibit no comparable axis preservation (Appendix \ref{sec: vit-alignment}), pointing to a fundamental architectural split: CNNs converge on a shared neuron-level coordinate system, whereas ViTs organise features in a basis that varies across runs.  

\paragraph{Hierarchical correspondence holds across metrics.}
\label{par: inter-network}
%\input{8pager/figures-code/inter-model-proc}
%\input{./figures-code/inter-model-sm}
Previous studies have shown that for architecturally identical networks trained from different initializations, the layer most similar to a given layer in another network is the corresponding architectural layer~\citep{kornblith2019similarity}. However, this finding has primarily been supported using metrics invariant to affine transformations (\emph{e.g.,} CCA, SVCCA). Here, we extend this result by showing that stricter metrics---such as Procrustes and soft-matching scores---also reveal the same hierarchical correspondence (Fig.~\ref{tab:procrustes_inter_model}), even when comparing networks with different architectures. This suggests that the hierarchical alignment of representations is a fundamental property of neural networks, robust to both architectural differences and the choice of alignment metric. Moreover, our results show that both representational shape (captured by Procrustes) and neuron-level tuning (captured by soft-matching) follow similar alignment patterns, reinforcing the consistency of this hierarchical organization across different levels of representational analysis.
%Previous studies have shown that, for architecturally identical networks trained from different initializations, the most similar layer in one network to a given layer in another is the corresponding architectural layer~\citep{kornblith2019similarity}. However, this finding has primarily been supported using metrics invariant to affine transformations (\emph{e.g.,} CCA, SVCCA). Here, we extend this result by showing that stricter metrics---such as Procrustes and soft-matching scores---also reveal the same hierarchical correspondence (Figs.~\ref{tab:procrustes_inter_model}, ~\ref{tab:sm_inter_model}), even when comparing networks with different architectures. This suggests that the hierarchical alignment of representations is a fundamental property of neural networks, robust to both architectural differences and the choice of alignment metric. Moreover, our results show that both representational shape (captured by Procrustes) and neuron-level tuning (captured by soft-matching) follow similar alignment patterns, reinforcing the consistency of this hierarchical organization across different levels of representational analysis.

==> yztwgkssnyyscymchgzppyswgzfcqwzw/acrosstraining.tex <==
\subsection{Evolution of convergence over training}
\label{sec: convergence-dynamics}
We next explore how representational convergence evolves during the training process. Specifically, we compute Procrustes alignment scores between pairs of networks over training epochs.
% training evo
\input{./figures-code/training-evo}
As shown in Fig.~\ref{fig:training-evo}, a striking pattern emerges: the majority of representational convergence occurs within the first epoch---long before a networks task performance peaks. This rapid early convergence suggests that factors independent of task optimization drive much of the representational alignment (see also Appendix~\ref{sec: training-rep-trained}). Shared input statistics, architectural biases, and early training dynamics seem to play a dominant role in shaping representational convergence, overshadowing the influence of the final task-specific solution.
%As shown in Fig.~\ref{fig:training-evo}, a striking pattern emerges: the majority of representational convergence occurs within the first epoch---long before networks approach optimal task performance. This rapid early convergence suggests that factors independent of task optimization drive much of the representational alignment. Shared input statistics, architectural biases, and early training dynamics seem to play a dominant role in shaping learned representations, overshadowing the influence of the final task-specific solution.
This observation challenges prevailing hypotheses, such as the \emph{contravariance principle}~\citep{cao2021explanatory} and \emph{task generality hypothesis}~\citep{huh2024platonic}, which argue that networks align because only a narrow solution subspace yields high performance. Instead, our findings point to inductive biases and early learning processes as the dominant forces shaping representational convergence.
%This observation challenges prevailing hypotheses that attribute convergence to task constraints, such as the \emph{contravariance principle}~\citep{cao2021explanatory} and \emph{task generality hypothesis}~\citep{huh2024platonic}, which posits that networks converge towards a limited subspace of solutions capable of achieving high task performance. However, the early emergence of representational alignment---well before high task accuracies---implies that convergence is instead driven by inductive biases, input statistics, and early training dynamics.

%Our early training convergence parallels the \emph{``silent alignment''} effect~\citep{atanasov2021neural}---networks can align with the target function early in training, before significant loss reduction. However, a key difference is that they study output-level alignment while we examine internal representations across different models.
%Our observed early alignment is consistent with the \emph{``silent alignment''} effect~\citep{atanasov2021neural}, where networks align with the target function early in training, before significant loss reduction. However a key difference is that they study output-level alignment while we examine internal representations across different models.

Our findings echo those of~\citep{frankle2020early}, who showed that most representational re-organization happens within the first few hundred iterations---well before any substantive task learning. Perturbing weights during this brief window (by re-initializing or shuffling them) severely impairs eventual accuracy, indicating the formation of early, data-dependent structure. Together, these observations reinforce the view that shared input statistics—not task labels---are the principal drivers of early representational convergence.

% These results align with ~\citep{frankle2020early}, who demonstrated that substantial changes in network representations occur in the first few hundred iterations, before meaningful task learning begins. Their work showed that perturbations to network weights in this early phase---such as re-initialization or weight shuffling---can significantly degrade performance, suggesting early structured, data-dependent representations. Moreover, they found that pre-training using only the input distribution \emph{p(x)} (\emph{e.g.,} through self-supervised tasks) could approximate the changes seen in early supervised training, albeit requiring substantially longer pre-training. This also lends credence to the idea that shared input statistics, rather than task-specific labels, play a critical role in early convergence.

%Interestingly, this result \textcolor{red}{also} aligns with findings from another study on the early phase of training~\citep{frankle2020early}, which demonstrated that substantial changes in network representations occur within the first few hundred iterations, even before meaningful task learning begins. Their work showed that perturbations to network weights in this early phase---such as re-initialization or weight shuffling---can significantly degrade performance, suggesting that early representations are already highly structured and data-dependent. Moreover, they found that pre-training using only the input distribution \emph{p(x)} (\emph{e.g.,} through self-supervised tasks) could approximate the changes seen in early supervised training, albeit requiring substantially longer pre-training. This also lends credence to the idea that shared input statistics, rather than task-specific labels, play a critical role in early convergence.
Early convolutional layers show little training-induced change on representational similarity (even reducing in some cases). This phenomenon arises because early layers compute near-linear mappings of the input, even in untrained networks, allowing them to align well with simple linear transformations. Subsequent training only makes minor adjustments that slightly disrupt initial alignment, though they remain highly similar overall. 
%This result highlights that the convergence of early-layer representations is not driven by the specifics of the training process. 
%For the earliest convolutional layers, we find that training has minimal impact on representational similarity and can even reduce it in some cases. This phenomenon arises because early layers compute a largely linear function of the input, even in untrained networks, allowing them to align well with simple linear transformations. As training progresses, these layers may undergo minor adjustments that slightly disrupt this initial alignment, though they remain highly similar overall. This result highlights that the convergence of early-layer representations is not driven by the specifics of the training process. 


==> yztwgkssnyyscymchgzppyswgzfcqwzw/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} 
    \item[] Justification: Yes, we have described these in the discussion section.
    
\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} 
    \item[] Justification: No theoretical results are discussed in this paper.
    
    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} 
    \item[] Justification: Yes, we discuss our experimental setup in both Section 3 and Appendix A1.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} 
    \item[] Justification: All datasets are publicly available. We provide a link to our code in the Supplementary section.
    
\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, we describe these details in Appendix A1.
    
\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} 
    \item[] Justification: Yes, they are displayed in all figures.
    
\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} 
    \item[] Justification: Yes, all models and subsequent analyses were performed on an NVIDIA A40 GPU. Training an ImageNet model took $\approx 80$ hours and CIFAR100 models took $\approx 4$ hours. 
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} 

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} 
    \item[] Justification: We don't foresee any negative societal impact of our work.
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} 
    \item[] Justification: In our knowledge, we don't use any model that may pose a risk for misuse.
    
\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} 
    \item[] Justification: Yes (\emph{e.g.,}~\cite{deng2009imagenet},~\cite{geirhos2018imagenet})

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No new assets are introduced in this paper.
    
\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    
\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} 
    
\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} 
    \item[] Justification: We didn't use LLMs to conduct any original scientific work or hypotheses.
    
\end{enumerate}



==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/inter-model-cifar100.tex <==
\begin{figure*}[htbp!]
    \centering
    % procrustes
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/resnet18_resnet50_orthogonal_procrustes_cifar100_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/resnet18_vgg16_orthogonal_procrustes_cifar100_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/resnet18_vgg19_orthogonal_procrustes_cifar100_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/vgg16_resnet50_orthogonal_procrustes_cifar100_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/vgg19_resnet50_orthogonal_procrustes_cifar100_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/vgg16_vgg19_orthogonal_procrustes_cifar100_comparison.png}\\
    
    % soft-match
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/resnet18_resnet50_soft_match_cifar100_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/resnet18_vgg16_soft_match_cifar100_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/resnet18_vgg19_soft_match_cifar100_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/vgg16_resnet50_soft_match_cifar100_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/vgg19_resnet50_soft_match_cifar100_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/vgg16_vgg19_soft_match_cifar100_comparison.png}
    
    \caption{\textbf{Inter-Model Comparisons on CIFAR100.} We consider all pairs of vision models, and compute the alignment scores between every pair of layers using the orthogonal Procrustes (\textbf{Top}) and Soft-Matching (\textbf{Bottom}) metric trained on CIFAR100. Gray line plots denote the maximum alignment value for each network over rows and columns.}%We consider all pairs of vision models, and for each pair, compute the alignment scores between every pair of layers using the orthogonal Procrustes metric trained on ImageNet. Gray line plots denote the \textbf{maximum} alignment value for each network over rows (right line) and columns (top line). A common trend that is observed here is the consistent relationships between layers of CNNs trained with different architectures.}
    \label{tab:procrustes_inter_model}
\end{figure*}

==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/inter-model-comparisons.tex <==
\begin{figure*}[htbp!]
    \centering
    % procrustes
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_resnet50_orthogonal_procrustes_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg16_orthogonal_procrustes_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg19_orthogonal_procrustes_imagenet_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet50_vgg16_orthogonal_procrustes_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet50_vgg19_orthogonal_procrustes_imagenet_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/vgg16_vgg19_orthogonal_procrustes_imagenet_comparison.png}\\

    % soft-matching
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_resnet50_soft_match_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg16_soft_match_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg19_soft_match_imagenet_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/resnet50_vgg16_soft_match_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet50_vgg19_soft_match_imagenet_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/vgg16_vgg19_soft_match_imagenet_comparison.png}
    
    \caption{\textbf{Inter-Model Comparisons.} We consider all pairs of vision models, and for each pair, compute the alignment scores between every pair of layers using the orthogonal Procrustes (\textbf{Top}) and Soft-Matching (\textbf{Bottom}) metric trained on ImageNet. Gray line plots denote the \textbf{maximum} alignment value for each network over rows (right line) and columns (top line). A common trend that is observed here is the consistent relationships between layers of CNNs trained with different architectures.}
    \label{tab:procrustes_inter_model}
\end{figure*}

==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/inter-model-sm.tex <==
\begin{figure}[htbp!]
    \centering
    % cifar100
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_resnet50_soft_match_cifar100_comparison.png}\hfill
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg16_soft_match_cifar100_comparison.png}\hfill
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg19_soft_match_cifar100_comparison.png}\hfill 
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/vgg16_resnet50_soft_match_cifar100_comparison.png}\hfill
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/vgg19_resnet50_soft_match_cifar100_comparison.png}\hfill 
    %\includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/vgg16_vgg19_soft_match_cifar100_comparison.png}\\
    
    % imagenet
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_resnet50_soft_match_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg16_soft_match_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet18_vgg19_soft_match_imagenet_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{./figures/inter-model-analysis-results/resnet50_vgg16_soft_match_imagenet_comparison.png}\hfill
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/resnet50_vgg19_soft_match_imagenet_comparison.png}\hfill 
    \includegraphics[width=.16\textwidth]{figures/inter-model-analysis-results/vgg16_vgg19_soft_match_imagenet_comparison.png}
    \caption{\textbf{Inter-Model Soft-Match.} Identical to the preceding plot, we compute the layer-wise soft-matching score for all networks pairs ImageNet, similarly revealing consistent inter-layer relationships across architectures.}
    
    \label{tab:sm_inter_model} 
\end{figure}

==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/language.tex <==
\begin{figure*}[t]%[!htbp]
    \centering
    %\includegraphics[scale=0.5]{./figures/language/pythia_res.png}
    \includegraphics[width=0.85\textwidth]{./figures/language/pythia_res.png}
    \caption{\textbf{Representational Convergence in Language Models.} \textbf{(A)} Alignment scores across all layers for Pythia-160m models trained from different seeds evaluated on STSB. \textcolor{mplorange}{Procrustes} align representations nearly as well as \textcolor{mplblue}{linear} transformations, mimicking the trend observed for vision models. \textbf{(B)} We compute the alignment scores using the Procrustes metric for every pair of layer in a seed-pair of Pythia-160m models. \textbf{(C)} Same as \textbf{(B)}, but for models with different architectures (varying depth). \textbf{(D)} Procrustes alignment between model pairs over training checkpoints.}
    %\caption{\textbf{Representational Convergence in Language Models.} \textbf{(A)} Alignment scores across all layers for Pythia-160m models trained from different seeds, evaluated on the Semantic Textual Similarity Benchmark~\citep{cer2017semeval}. Alignment consistently follows the order \textcolor{mplblue}{Linear} $>$ \textcolor{mplorange}{Procrustes} $>$ \textcolor{mplgreen}{Permutation}. \textcolor{mplorange}{Procrustes} align representations nearly as well as \textcolor{mplblue}{Linear} transformations, mimicking the trend observed for vision model. \textbf{(B)} We compute the alignment scores using the Procrustes metric for every pair of layer in a seed-pair of Pythia-160m models. \textbf{(C)} Same as \textbf{(B)}, but for models with different architectures (varying depth). \textbf{(D)} Procrustes alignment between model pairs over training checkpoints: alignment peaks early ($\approx 8-10$B tokens) and then plateaus or decreases even as next-token prediction accuracy continues to improve.}
    %\caption{\textbf{Representational convergence in Language Models.} \textbf{(A)} We plot the evolution of alignment scores (computed between different seeds of the same network architecture) across the network hierarchy for language models (Pythia-$160$m) trained with different seeds on the same Pile dataset. The alignment values are computed using all sentences from the Semantic Textual Similarity Benchmark~\citep{cer2017semeval}. Alignment consistently follows the order: \textcolor{mplblue}{Linear} $>$ \textcolor{mplorange}{Procrustes} $>$ \textcolor{mplgreen}{Permutation}, reflecting the progressively stricter nature of the metrics. Notably, \textcolor{mplorange}{Procrustes} transformations align representations nearly as well as \textcolor{mplblue}{Linear} transformations, mimicking the trend observed for vision models. \textbf{(B)}. \textbf{Inter-Model Orthogonal Procrustes.} We consider pairs of Pythia-$160$m models trained on different seeds, and for each pair, compute the alignment scores between every pair of layers using the orthogonal Procrustes metric. \textbf{(C)} Same as \textbf{B} but computed between networks with different architectures (specifically layer depths). \textbf{(D)} We visualize the evolution of Procrustes alignment between network pairs during across different model checkpoints. Alignment peaks around rapidly $8-10$B tokens before saturating or declining even though the next-word prediction performance continues to improve.}
    \label{fig:lang}
\end{figure*}

==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/network-hierarchy.tex <==
\begin{figure*}[htbp!]
    \centering
    % cifar100
    %\includegraphics[width=.25\textwidth]{figures/network-hierarchy/r18_cifar100.png}\hfill
    %\includegraphics[width=.25\textwidth]{figures/network-hierarchy/r50_cifar100.png}\hfill
    %\includegraphics[width=.25\textwidth]{figures/network-hierarchy/vgg16_cifar100.png}\hfill
    %\includegraphics[width=.25\textwidth]{figures/network-hierarchy/vgg19_cifar100.png}\\
    % imagenet
    \includegraphics[width=.25\textwidth]{./figures/network-hierarchy/r18_imagenet_untrained.png}\hfill
    \includegraphics[width=.25\textwidth]{./figures/network-hierarchy/r50_imagenet_untrained.png}\hfill
    \includegraphics[width=.25\textwidth]{./figures/network-hierarchy/vgg16_imagenet_untrained.png}\hfill
    \includegraphics[width=.25\textwidth]{./figures/network-hierarchy/vgg19_imagenet_untrained.png}
    
    \caption{\textbf{Representational Convergence Across a Network Hierarchy.} We plot the evolution of alignment scores (computed between different seeds of the same network architecture) across the network hierarchy for four vision network architectures trained ImageNet. A consistent downward trend across layers indicates decreasing representational convergence as networks deepen. Alignment consistently follows the order: \textcolor{mplblue}{Linear} $>$ \textcolor{mplorange}{Procrustes} $>$ \textcolor{mplgreen}{Permutation}, reflecting the progressively stricter nature of the metrics. Lighter shades of the same color denote alignment for random networks. Notably, \textcolor{mplorange}{Procrustes} transformations align representations nearly as well as \textcolor{mplblue}{Linear} transformations, suggesting that most variability is due to rotations rather than more complex transformations. Even \textcolor{mplgreen}{Permutation} scores---despite their strictness---achieve substantial alignment, indicating a strong one-to-one correspondence between neurons across seeds, which points to stable, convergent neuron-level representations. Error bars represent the standard deviation computed across $5$-fold cross-validation.}
    \label{fig:network-hierarchy}
\end{figure*}


==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/ood-amplification-swav.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{8pager/figures/nsd-results/self-supervised.png}
    \caption{Caption}
    \label{fig:ood-amplification-swav}
\end{figure}

==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/ood-amplification.tex <==
%\begin{figure}
%    \centering
%    \includegraphics[scale=0.33]{figures/ood-divergence/ood_amplification.png}
%    \caption{\textbf{Amplifying Model Differences.}}
%    \label{fig:enter-label}
%\end{figure}

\begin{figure}[htbp!]
    \centering
    \includegraphics[width=\textwidth]{figures/ood-divergence/ood_amplification.png}
    \caption{\textbf{Procrustes Score-based Alignment Between Networks Sharing the Same Architecture but Trained With Different Random Seeds, Plotted as a Function of Layer Depth.} Alignment is measured using within-distribution (WD) stimuli (ImageNet test set) and out-of-distribution (OOD) stimuli, with OOD values averaged across $17$ datasets. Error bars represent the standard error computed across the $(n = 17)$ OOD datasets.}
    \label{fig:ood-amplification}
\end{figure}


==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/ood-imagenet.tex <==
\begin{figure*}[htbp!]
    \resizebox{\textwidth}{!}{
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=0.5\textwidth]{figures/ood-divergence/resnet18_ood_divergence.png} &      
        \includegraphics[width=0.5\textwidth]{figures/ood-divergence/vgg16_ood_divergence.png} \\
        \textbf{(a)} ResNet18 & \textbf{(b)} VGG16 \\
        \multicolumn{2}{c}{\includegraphics[width=0.5\textwidth]{figures/ood-divergence/vgg19_ood_divergence.png}} \\
        \multicolumn{2}{c}{\textbf{(c)} VGG19}
    \end{tabular}
    }
    \caption{\textbf{Procrustes Alignment vs. Task Performance} We compute the Procrustes alignment of different network architectures on each of the $17$ datasets for the first convolutional layer \textbf{(Left)} and the penultimate \textbf{(Right)} layer from \textbf{(a)} - \textbf{(c)}.}
    \label{fig:ood-convergence-appendix}
\end{figure*}


==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/pearson-ood.tex <==
%\begin{figure}
%    \centering
%    \includegraphics[scale=0.5]{figures/ood-divergence/pearson_ood_all_layers.png}
%    \caption{\textbf{Pearson Correlation Across Network Hierarchy.}}
%    \label{fig: corr-ood-network-hierarchy}
%\end{figure}

\begin{figure*}[htbp!]
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cc}
        \raisebox{0.5cm}{
        \includegraphics[height=0.15\textheight]{figures/ood-divergence/resnet50_ood_divergence.png}%
        }
        & \includegraphics[width=0.4\textwidth]{./figures/ood-divergence/pearson_ood_all_layers.png}\\
    \textbf{(a)} & \textbf{(b)} 
    \end{tabular}
    }
    \caption{\textbf{Convergence on OOD Inputs.} \textbf{(a)} Procrustes alignment vs. task performance of ResNet$50$ models on each of the $17$ datasets for the first convolutional layer \textbf{(Left)} and the penultimate \textbf{(Right)} layer. \textbf{(b)} Correlation between these variables as a function of network depth (normalized by each models depth). 
    % Here, the error bars represent the standard deviation of $r$ after excluding one dataset at a time (i.e., using $n=16$ remaining datasets).
    }
    \label{fig: ood-convergence}
\end{figure*}    

==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/privileged-axes-table.tex <==
%\begin{table}[htbp!]
%    \centering
%    \resizebox{\textwidth}{!}{
%    \begin{tabular}{cccc}
%    \toprule
%    Model & Native (Min / Max) & Rotated (Min / Max) & Difference ($\%$) (Min / Max)\\
%    \midrule
%        %ResNet18 (CIFAR100) & $0.247 \ / \ 0.752$ & $0.215 \ / \ 0.689$ & $6.40\% \ / \ 51.26\%$ \\
%        %ResNet50 (CIFAR100) & $0.254 \ / \ 0.828$ & $0.242 \ / \ 0.828$ & $-3.38\% \ / \ 35.29\%$ \\
%        %VGG16 (CIFAR100) & $0.277 \ / \ 0.769$ & $0.239 \ / \ 0.661$ & $5.66\% \ / \ 63.97\%$ \\
%        %VGG19 (CIFAR100) & $0.273 \ / \ 0.758$ & $0.231 \ / \ 0.684$ & $2.15\% \ / \ 35.36\%$ \\
%        ResNet18 & $0.202 \ / \ 0.721$ & $0.154 \ / \ 0.581$ & $10.47\% \ / \ 201.84\%$ \\
%        ResNet50 & $0.225 \ / \ 0.791$ & $0.143 \ / \ 0.739$ & $2.61\% \ / \ 180.75\%$ \\
%        VGG16 & $0.288 \ / \ 0.746$ & $0.181 \ / \ 0.599$ & $21.72\% \ / \ 81.12\%$ \\
%        VGG19 & $0.292 \ / \ 0.799$ & $0.171 \ / \ 0.562$ & $41.95\% \ / \ 89.68\%$ \\
%    \bottomrule
%    \end{tabular}
%    }
%    \vspace*{0.5em}
%    \caption{\textbf{Sensitivity of Permutation Scores to Representational Axes.} \textcolor{red}{For each ImageNet-trained network we apply a random rotation to the network’s unit basis, recompute permutation-based alignment scores, and summarize the results across convolutional layers. Columns report the minimum and maximum alignment scores observed over layers in the native basis and in the rotated basis. The final column gives the percentage change in alignment after rotation. Rotations almost always reduce alignment, indicating the distinguished nature of the representational axes for all layers in networks.}}
%    
%    %We rotate the native axes for each of the ImageNet-trained networks by a random rotation matrix and recompute alignment scores. We report the min / max alignment scores across all layers for the alignment in the native and rotated bases and observe that rotations almost always reduce the alignment score, highlighting the distinguished nature of the representational axes for all layers in networks.}
%    \label{tab:perm-rotated}   
%\end{table}


\begin{wraptable}{r}{8cm}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{cccc}
        \toprule
        Model & Native (Min / Max) & Rotated (Min / Max) & Difference ($\%$) (Min / Max)\\
        \midrule
            ResNet18 & $0.202 \ / \ 0.721$ & $0.154 \ / \ 0.581$ & $10.47\% \ / \ 201.84\%$ \\
            ResNet50 & $0.225 \ / \ 0.791$ & $0.143 \ / \ 0.739$ & $2.61\% \ / \ 180.75\%$ \\
            VGG16 & $0.288 \ / \ 0.746$ & $0.181 \ / \ 0.599$ & $21.72\% \ / \ 81.12\%$ \\
            VGG19 & $0.292 \ / \ 0.799$ & $0.171 \ / \ 0.562$ & $41.95\% \ / \ 89.68\%$ \\
        \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Sensitivity of Permutation Scores to Representational Axes.} For each ImageNet-trained network we apply a random rotation to the network’s unit basis, recompute permutation-based alignment scores, and summarize the results across convolutional layers. Columns report the minimum and maximum alignment scores observed over layers in the native basis and in the rotated basis. The final column gives the percentage change in alignment after rotation. Rotations almost always reduce alignment, indicating the distinguished nature of the representational axes for all layers in networks.}
    \label{tab:perm-rotated}
\end{wraptable}


==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/random-pixel-hierarchy.tex <==
\begin{figure*}[htbp!]
    \centering
    \includegraphics[width=.25\textwidth]{figures/random-pixel/hierarchy/r18_imagenet_random_pixel.png}\hfill
    \includegraphics[width=.25\textwidth]{figures/random-pixel/hierarchy/r50_imagenet_random_pixel.png}\hfill
    \includegraphics[width=.25\textwidth]{figures/random-pixel/hierarchy/vgg16_imagenet_random_pixel.png}\hfill
    \includegraphics[width=.25\textwidth]{figures/random-pixel/hierarchy/vgg19_imagenet_random_pixel.png}
    
    \caption{\textbf{Representational Convergence Across a Network Hierarchy Using a Random Pixel.} We plot the representational convergence across (ImageNet-trained) network hierarchies using both---the central pixel (darker shade) and a random pixel (lighter shade) for $3$ alignment metrics---\textcolor{mplblue}{Linear predictivity}, \textcolor{mplorange}{Procrustes}, \textcolor{mplgreen}{Permutation}. Across all these metrics, we observe that the spatial choice of the sample pixel leaves the alignment effectively unchanged.}
    \label{fig:network-hierarchy-random-pixel}
\end{figure*}


==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/self-supervised.tex <==
\begin{figure}[htbp!]
    \centering
    \includegraphics[width=\textwidth]{./figures/self-supervised/moco.png}
    \caption{\textbf{Representational Alignment with Self-Supervised Networks.} \textbf{(A)} Representational alignment across layers of a pair of MoCo-trained ResNet$50$ models on ImageNet. Error bars indicate standard deviation from $5$-fold cross-validation. \textbf{(B)} We plot the Procrustes alignment between MoCo models evaluated on in-distribution (ImageNet) and out-of-distribution (Stylized ImageNet~\citep{geirhos2018imagenet}) stimuli. Error bars show standard error across all $(n=17)$ OOD datasets. \textbf{(C)} Change in Procrustes alignment score with every training epoch. Colors in the bar-plot indicate the top-$1$ accuracies during training. \textbf{(D)} Permutation alignment in the native and randomly rotated basis. Each dot corresponds to a convolutional ResNet$50$ layer. Bars indicate mean alignment. Rotation reduces mean alignment by $14.87\%$.}
    \label{fig:self-supervised}
\end{figure}


==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/spearman.tex <==
\begin{figure*}[htbp!]
    \centering
    \includegraphics[width=.25\textwidth]{./figures/spearman-correlation/r18_imagenet_spearman.png}\hfill
    \includegraphics[width=.25\textwidth]{./figures/spearman-correlation/r50_imagenet_spearman.png}\hfill
    \includegraphics[width=.25\textwidth]{./figures/spearman-correlation/vgg16_imagenet_spearman.png}\hfill
    \includegraphics[width=.25\textwidth]{./figures/spearman-correlation/vgg19_imagenet_spearman.png}
    
    \caption{\textbf{Representational Convergence Across a Network Hierarchy Using Spearman's Rank Correlation.} We plot the evolution of alignment scores computed between different (ImageNet-trained) network seeds of the same architecture. Lighter shades of the same color denote the Spearman's ranked-correlation score, whereas darker shades indicates the Pearson correlation-based alignment score. We clearly observe that both correlation measures yield nearly identical results.}
    \label{fig:network-hierarchy-spearman}
\end{figure*}


==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/swav-hierarchy.tex <==
\begin{figure*}[htbp!]
    \centering
    \includegraphics[scale=0.5]{8pager/figures/network-hierarchy/r50_swav_imagenet.png}
    \caption{\textbf{Representational Convergence Across Network Hierarchy Using SwAV Training.} We evaluate representational alignment for a pair of SwAV-trained, ResNet50 backbone network on the ImageNet dataset. Error bars denote the standard deviation computed across 5-fold cross-validation.}
    \label{fig:swav-hierarchy}
\end{figure*}

==> yztwgkssnyyscymchgzppyswgzfcqwzw/figures-code/training-evo.tex <==
\begin{figure*}[htbp!]
    \centering
    %\includegraphics[width=0.9\textwidth]{./figures/training-evo/self-supervised.png}
    %\includegraphics[width=0.6\textwidth]{./figures/training-evo/cifar100_training_evo_all_pairs.png}
    \includegraphics[width=\textwidth]{./figures/training-evo/imagenet_training_evo_all_pairs.png}
    \caption{\textbf{Representational Alignment Through Training Evolution.}  We visualize the evolution of Procrustes alignment between network pairs during task optimization on ImageNet. Lighter shades indicate earlier epochs, progressively darkening with later epochs. The plots span from epoch $0$ (untrained) to epoch $10$, with task performance improving over time. Epoch progression can be inferred from the increasing task performance along the $x$-axis.}
    \label{fig:training-evo}
\end{figure*}

==> yztwgkssnyyscymchgzppyswgzfcqwzw/intro.tex <==
Deep Neural Networks (DNNs) are becoming increasingly popular in neuroscience for predicting neural responses~\citep{yamins2014performance, yamins2016using, khaligh2014deep}, or as models for reverse-engineering algorithms of neural computation~\citep{schrimpf2018brain, schrimpf2020integrative, cichy2016comparison}. This congruence invokes the necessity to gain a deep understanding of how DNNs learn to represent information. A core question in this domain is whether independently trained networks converge on similar internal representations---and if so, under what conditions and along which dimensions this convergence unfolds? Comparative analysis of model representations helps reverse engineering neural networks by linking architectural components, training objectives, and data inputs to learned representations and, in turn, model behavior.
%Deep Neural Networks (DNNs) are becoming increasingly popular in neuroscience for predicting neural responses~\citep{yamins2014performance, yamins2016using, khaligh2014deep}, or as models for reverse-engineering algorithms of neural computation~\citep{schrimpf2018brain, schrimpf2020integrative, cichy2016comparison}. This congruence invokes the necessity to gain a deep understanding of how DNNs learn to represent information. A core question in this domain is whether independently trained networks converge on similar internal representations---and if so, under what conditions and along which dimensions this convergence unfolds? Comparative analysis of model representations helps reverse engineering neural networks by linking architectural components, training objectives, and data inputs to learned representations and, in turn, model behavior. For neuroscientific modeling using DNNs, a foundational question lies in ascertaining which aspects of their representations vary across different architectural choices, and which aspects---if any---are universal across such choices. Thus, studying this representational convergence has far-reaching implications. 

Over the past decade, there has been growing recognition that similar representations emerge across diverse models, despite differing in architecture, training procedures, or data modalities. Early work demonstrated that independent training runs of the same architecture develop a core set of features that align well across networks. For example, early layers in convolutional networks learn Gabor-like filters, across a range of architectures and tasks~\citep{yosinski2014transferable, krizhevsky2012imagenet}. Efforts to quantify these similarities have employed techniques such as canonical correlation analysis (CCA) and its variants~\citep{morcos2018insights, raghu2017svcca}, centered kernel alignment (CKA)~\citep{kornblith2019similarity}, representational similarity analysis (RSA)~\citep{mehrer2020individual} and model stitching~\citep{bansal2021revisiting}. These studies have underscored the high degree of alignment in early layers and noted convergence even in later stages of the network. These findings provide empirical grounding for theories of representational convergence, hinting at the existence of universal principles governing learning, which may also shed light on how biological neural circuits process information.

%Over the past decade, there has been growing recognition that similar representations can emerge across diverse models, despite models differing in architecture, training procedures, or data modalities. Early work demonstrated that independent training runs of the same architecture develop a core set of features that align well across networks. For example, early layers in convolutional networks learn Gabor-like filters, across a range of architectures and tasks~\citep{yosinski2014transferable, krizhevsky2012imagenet}. Efforts to quantify these similarities have employed techniques such as canonical correlation analysis (CCA) and its variants~\citep{morcos2018insights, raghu2017svcca}, centered kernel alignment (CKA)~\citep{kornblith2019similarity}, representational similarity analysis (RSA)~\citep{mehrer2020individual} and model stitching~\citep{bansal2021revisiting}. These studies have underscored the high degree of alignment in early layers and noted convergence even in later stages of the network. These findings provide empirical grounding for theories of representational convergence, hinting at the existence of universal principles governing learning, which may also shed light on how biological neural circuits process information.

Recent studies have extended this line of inquiry, demonstrating that increasing model capability---through increased scale, multitask training, or cross-modal learning---drives representational convergence not just within, but also \emph{across} modalities~\citep{moschella2023relative}. The Platonic Representation Hypothesis further argues that as models scale and solve more tasks, they are driven to discover a universal, modality-agnostic representation of reality~\citep{huh2024platonic}. Yet, identifying precise conditions of network convergence on similar representations and its implications remain open questions.

%Recent studies have extended this line of inquiry, demonstrating that increasing model capability---through increased scale, multitask training, or cross-modal learning---their representations converge not only within a single modality, but also across modalities ~\citep{moschella2023relative}. For instance, the Platonic Representation Hypothesis argues that as models solve a larger number of tasks and scale up in capacity, they are pressured into discovering a universal, modality-agnostic representation of the underlying reality~\citep{huh2024platonic}. Yet, many open questions remain about the conditions under which different networks converge on similar representations and the implications of such convergence.
To address these gaps, in our work, we examine representational alignment along three key axes:\\
\newline
\textbf{Across layers:} %One important axis of inquiry is representational alignment across layers. Prior work has shown that early layers tend to extract general, low-level features---such as edge detectors in vision networks---while deeper layers develop more task-specific representations. Studies by~\citep{kornblith2019similarity},~\citep{mehrer2020individual}, and~\citep{li2015convergent} have quantified these changes using methods like canonical correlation analysis (CCA) and CKA. However, these approaches often rely on single metrics that obscure the minimal transformations needed to align representations. Understanding the precise nature of these transformations is critical for dissecting how representations in different networks relate to each other (\emph{e.g.}, are they similar in information content, representational geometry, or even at the level of single-neuron tuning?). It is also unknown whether the hierarchical (layer-wise correspondence) results hold true for other metrics with more restricted invariances than affine transformations.
Prior work has shown that early layers tend to extract general, low-level features---such as edge detectors in vision networks---while deeper layers develop task-specific representations. Studies~\citep{kornblith2019similarity, mehrer2020individual, li2015convergent} have quantified these changes using methods like CCA and CKA. However, these approaches often rely on single metrics that obscure minimal transformations needed to align representations. Understanding the precise nature of these transformations is critical for dissecting how representations in different networks relate to each other (\emph{e.g.}, are they similar in information content, representational geometry, or even at the level of single-neuron tuning?). It is also unknown whether hierarchical (layer-wise) correspondence holds for other metrics with more restricted invariances than affine transformations.\\
\newline
\textbf{Across training:} %A second key question concerns the evolution of representational convergence over the course of training. Most studies compare networks at their converged state. Yet, a deeper understanding requires examining not only the final representations, but also the learning trajectories that lead there. Conventionally, it is assumed that as different networks optimize on a task, their internal representations become more similar, driven by the final task solution. This assumption is the basis for the \emph{contravariance principle}~\citep{cao2021explanatory}, which posits that when a network is pushed to achieve a challenging task, there is less room for variation in the final solution, forcing representations to converge. However, the question of when representational convergence occurs \emph{during} training remains underexplored. Understanding this dynamic can illuminate the roles of initialization, early data statistics, architectural biases, learning dynamics, and the final task solution in shaping alignment. Previous studies have shown a \emph{``lower layers learn first''}~\citep{raghu2017svcca} behavior by comparing layers across time on CIFAR-10 using SVCCA, but little else is known about the dynamics of convergence, especially for more complex vision networks and using other metrics. Recent theoretical studies such as~\citep{domine2024lazy},~\citep{saxe2013exact} present an analytical framework for the temporal dynamics of learning in deep \emph{linear} networks, distinguishing an early \emph{``lazy''} phase, characterized by kernel regression dynamics~\citep{jacot2018neural}---from a subsequent \emph{``rich''} phase characterized by non-linear feature learning. While these models provide valuable insights into training dynamics and convergence in linear regimes, they fall short of fully explaining representational alignment in complex, non-linear architectures. Though deep linear models are instructive, further work is needed to elucidate how representational alignment develops in and generalizes to the rich, nonlinear regimes typical of contemporary neural networks.
A second key question is \emph{when} convergence emerges. Most studies snapshot networks only after training has finished, but revealing the mechanisms behind alignment demands tracking how representations co-evolve during training, not just examining the final state. Conventionally, it is assumed that as different networks optimize on a task, their internal representations become more similar, driven by the final task solution. This assumption is the basis for the \emph{contravariance principle}~\citep{cao2021explanatory}, which posits that when a network is pushed to achieve a difficult task, there is less room for variation in the final solution, forcing representations to converge. However, the question of when representational convergence occurs \emph{during} training remains underexplored. Understanding this dynamic can illuminate the roles of initialization, early data statistics, architectural biases, learning dynamics, and the final task solution in shaping alignment. Previous studies have shown a \emph{``lower layers learn first''}~\citep{raghu2017svcca} behavior by comparing layers over time on CIFAR-10 using SVCCA, but little is known about the dynamics of convergence, especially for complex vision networks and using other metrics. More recently, Atanasov et al.~\citep{atanasov2021neural} described a \emph{``silent alignment effect''} in which a network's output aligns with the target function early in training well before the loss falls. Theoretical studies such as~\citep{braun2025not, domine2024lazy, saxe2013exact} present an analytical framework for the temporal dynamics of learning in deep \emph{linear} networks, distinguishing an early \emph{``lazy''} phase, characterized by kernel regression dynamics~\citep{jacot2018neural}---from a subsequent \emph{``rich''} phase characterized by non-linear feature learning. While these models provide valuable insights into training dynamics and convergence in linear regimes, they fall short of fully explaining representational alignment in non-linear architectures. Though deep linear models provide valuable theoretical traction, further work is needed to elucidate how representational alignment develops and generalizes to the rich, non-linear regimes typical of contemporary DNNs.\\
\newline
\textbf{Across distribution shifts:} Although many DNNs exhibit highly human-like responses to in-distribution stimuli, there is mounting evidence that their responses can diverge dramatically under out-of-distribution (OOD) conditions~\citep{prasad2022exploring, geirhos2021partial, geirhos2018generalisation}. Despite this, the effect of OOD inputs on model-to-model representational convergence remains poorly understood. Exploring this axis is crucial for rigorously testing the universality of learned representations.\\
\newline

\textbf{Key contributions.}  In this work, we address these critical gaps by performing a large-scale systematic audit of representational convergence along these three axes. First, we employ three alignment metrics---linear regression~\citep{yamins2014performance, schrimpf2018brain, zhuang2021unsupervised, kubilius2019brain}, Procrustes analysis~\citep{sucholutsky2023getting, williams2021generalized}, and permutation-based methods~\citep{li2015convergent, khosla2024soft, khosla2024privileged}---each with different restrictions on the freedom of the mapping function, to identify the minimal set of transformations needed to align representations across networks reasonably well for each layer. This approach allows us to dissect how representations relate to each other, whether in terms of information content, representational geometry, or single-neuron tuning. Second, we examine the temporal dynamics of convergence during training, revealing that nearly all alignment occurs within the first epoch, challenging the assumption that convergence is tied to task-specific learning. Finally, we explore how changes in input statistics affect representational alignment across layers, demonstrating how OOD inputs differentially affect later versus early layers.  








==> yztwgkssnyyscymchgzppyswgzfcqwzw/language-models.tex <==
\subsection{Representational Convergence in Language Models}
\label{sec: lang-alignment}
We analyze representation convergence in language models using sentence embeddings from the Semantic Textual Similarity Benchmark (STSB)~\citep{cer2017semeval}. Our analyses include two primary comparisons: \textbf{(i) Same architecture:} multiple \textbf{Pythia-160m} instances differing only by random seed, allowing us to analyze variability in representational spaces solely from stochastic training factors \textbf{(ii) Cross-architecture:} \textbf{Pythia-70m} vs. \textbf{Pythia-160m}, to probe the effect of network depth on learned representations.
%In this section, we rigorously analyze representational convergence in different language models. Specifically, our analyses includes:
%\begin{itemize}
%    \item \textbf{Same-Architecture Comparisons:} We compare multiple instances of the \textbf{Pythia-160m} model, which share an identical architecture but differ in the initialization of random seeds. This allows us to assess the variability in representational spaces resulting solely from stochastic training factors.
%    \item \textbf{Cross-Architecture Comparisons:} In addition to seed variation, we compare models with different architectural configurations, namely the \textbf{Pythia-70m} and the \textbf{Pythia-160m} models. The primary architectural difference lies in network depth (i.e., number of layers), offering insights into how differences in model capacity and depth impact the learned representations.
%\end{itemize}

%\noindent
%All alignment metrics are computed using the representations of all unique sentences from the Semantic Textual Similarity Benchmark (STSB) dataset~\citep{cer2017semeval}.

\input{./figures-code/language}

\paragraph{Methodology.} For our representational similarity analysis, we perform two sets of computations: \textbf{(i) Final Checkpoint:} we compute the similarity between every pair of layers for all models at their final checkpoints using the same metrics as in the case of vision models (Linear, Procrustes, Permutation). \textbf{(ii) Intermediate Checkpoint:} across $154$ intermediate checkpoints, we analyze layer representations at normalized depths $0$ (beginning), $0.5$ (middle), $1$ (end) in the network. We track changes in the Procrustes similarity over training.

%\textbf{1. Final Checkpoint Analysis:}  
%For each model at its final checkpoint, we compute the similarity between every pair of layers using the three metrics used for vision models, namely the Permutation, Procrustes and Linear Alignment measures. 
%
%\textbf{2. Intermediate Checkpoint Analysis:}  
%Across the training run, we analyze 154 intermediate checkpoints sampled during the training process of the Pythia suite. At each checkpoint, for each model, we extract layer representations at normalized indices corresponding to the beginning $(0)$, middle $(0.5)$, and end $(1)$ of the network. The similarity between these layers is then computed using the \textbf{Procrustes} measure. \\
%
\noindent

\textbf{Results.} Comparing representations across language models reveals three key patterns: 
(1) \textbf{Metric-dependent alignment:} alignment follows \textcolor{mplblue}{Linear} $>$ \textcolor{mplorange}{Procrustes} $>$ \textcolor{mplgreen}{Permutation} (Fig.~\ref{fig:lang}-A); \textcolor{mplorange}{Procrustes} and \textcolor{mplblue}{Linear} scores are nearly identical, indicating that rotations/reflections explain most variability across models, and high alignment persists across layers. 
(2) \textbf{Hierarchical correspondence:} layers at similar depths align most closely both within (Fig.~\ref{fig:lang}-B) and across architectures (Fig.~\ref{fig:lang}-C). 
(3) \textbf{Rapid convergence:} alignment emerges early (layers at indices $0$, $0.5$, $1$), peaks around $8$–$10$B tokens, then plateaus or slightly declines (Fig.~\ref{fig:lang}-D) even as next-token prediction improves up to $300$B tokens~\citep{biderman2023pythia}.


% \textbf{Results.} Comparing representations across different language models yields several key insights:
% \begin{itemize}
%     \item \textbf{Metric-Dependent Alignment:}  
%     \textcolor{red}{The evolution of alignment scores follows the order \textcolor{mplblue}{Linear} $>$ \textcolor{mplorange}{Procrustes} $>$ \textcolor{mplgreen}{Permutation}, as shown in Fig.~\ref{fig:lang}-A. \textcolor{mplorange}{Procrustes} and \textcolor{mplblue}{linear} alignment scores are nearly identical like vision models, again, indicating that rotations/reflections account for most of the variability across different language models. Unlike the vision models, high alignment is maintained across the network hierarchy.}
%     %As shown in Figure~\ref{fig:lang}-A, the evolution of alignment scores across the network hierarchy reveals that linear alignment consistently yields higher similarity scores compared to the Procrustes measure, which in turn scores higher than the permutation metric. However, as observed with vision networks, the Procrustes alignment approaches the linear alignment score  implying that simple rotational and reflectional transformations account for much of the variability in representations across different language models. Further, unlike the vision case, high alignment is maintained across the network hierarchy and does not diminish with network depth. 
%     \item \textbf{Hierarchical correspondence}: 
%     \textcolor{red}{Layer-wise alignment reveals a pattern analogous to vision, where layers at identical depths correspond most closely with one another---both within (Fig.~\ref{fig:lang}-B) and across architectures (Fig.~\ref{fig:lang}-C).}
%     %Layer-wise alignment comparisons reveal a pattern analogous to the one observed in vision models: early layers correspond most closely with early layers, mid-level layers with mid-level ones, and late layers with their counterparts. This systematic correspondence is evident both---for models sharing the same architecture (Figure~\ref{fig:lang}-B) and for models with different architectures (Figure~\ref{fig:lang}-C).
%     \item \textbf{Rapid representational convergence}  
%     \textcolor{red}{Representational alignment emerges early for all key layers (normalized indices $0$, $0.5$, $1$), and peaks near $\approx8-10$ billion tokens, then saturates or even slightly declines  (Fig.~\ref{fig:lang}-D) even as next-token prediction performance continues to improve up to $300$B tokens~\citep{biderman2023pythia}, mirroring the evolution observed in vision models.}
%     %An examination of intermediate checkpoints shows that representational alignment emerges early for all three key layers (normalized indices $0$, $0.5$, and $1$). Alignment scores generally peak at around $8-10$ billion tokens (Figure~\ref{fig:lang}-D), after which they stabilize or decline slightly---even as next-word prediction performance continues to improve up to $300$B tokens as reported in the Pythia paper~\citep{biderman2023pythia}. This mirrors the evolution observed in vision models.
% \end{itemize}


==> yztwgkssnyyscymchgzppyswgzfcqwzw/self-supervised.tex <==
\subsection{Representational Alignment for Self-Supervised Networks}
\label{sec: self-sup-alignment}

We next test whether our findings generalize to self-supervised learning. All analyses were replicated on models trained with a Momentum Contrast (MoCo) objective~\citep{he2020momentum} (training details in Appendix~\ref{sec: network-training}). 
(1) \textbf{Across hierarchy:} convergence is strongest in early layers and tapers with depth (Fig.~\ref{fig:self-supervised}-A); \textcolor{mplblue}{Linear} and \textcolor{mplorange}{Procrustes} scores remain comparable, suggesting inter-model variability reflects rotations/reflections. 
(2) \textbf{Across distribution shifts:} early layers maintain alignment for both in-distribution and OOD inputs, while deeper layers diverge (Fig.~\ref{fig:self-supervised}-B), indicating that self-supervised training, like supervised learning, produces stable, general early filters and increasingly distribution-sensitive higher representations.
(3) \textbf{Across training:} most alignment emerges within the first epoch, well before optimal task performance (Fig.~\ref{fig:self-supervised}-C). 
(4) \textbf{Permutation sensitivity:} applying a random rotation substantially reduces permutation alignment (Fig.~\ref{fig:self-supervised}-D), confirming convergence to a privileged basis regardless of learning paradigm.

% \textcolor{red}{We next test our findings on networks trained using a self-supervised learning objective. In particular, we replicate all our analyses on models trained with a Momentum Contrast (MoCo) objective~\citep{he2020momentum} (training details in Appendix~\ref{sec: network-training}).}
% %So far, we have demonstrated our findings using a fully supervised learning objective. To assess whether these findings generalize to alternative training paradigms, we next investigate the effect of a self-supervised learning approach. In particular, we validate our results on models trained with an unsupervised framework using a contrastive learning objective---Momentum Contrast (MoCo)~\citep{he2020momentum}, with architectural details in Appendix~\ref{sec: network-training}. 



% \paragraph{Alignment Across Network Hierarchy.}
% \textcolor{red}{Much like supervised models, representational convergence is strongest in early layers and tapers with depth (Fig.~\ref{fig:self-supervised}-A). An analogous trend follows---linear and Procrustes scores remain comparable, indicating that inter-model variability is largely captured by rotations/reflections rather than general affine maps.}
% %Much like fully supervised networks, our results indicate that representational convergence is most pronounced in early layers and decreases with network depth (Fig.~\ref{fig:self-supervised}-A). We also note an analogous trend of the linear and Procrustes alignment scores being comparable, suggesting that representational variability across models that can be explained well using rotations and reflections, rather than complex affine transformations.

% \paragraph{Convergence Across Distribution Shifts.} 
% \textcolor{red}{Early layers of MoCo models retain similar alignment for both in-distribution and OOD inputs, while deeper layers diverge under OOD stimuli (Fig.~\ref{fig:self-supervised}-B), indicating shared representational structure invariant to distribution shifts. This echoes are findings from supervised networks---self-supervised training also develops general, stable early filters and progressively more distribution-sensitive representations.}
% %When comparing representational alignment between self-supervised networks across distribution shifts, we observe that OOD and in-distribution alignment values are closely matched in early layers, indicating shared representational structure robust to distribution shifts. In contrast, deeper layers show increasing divergence (Fig.\ref{fig:self-supervised}-B) for OOD inputs. This echoes our findings from supervised networks---even under self-supervised learning, networks initially develop general-purpose filters that are fairly aligned across all stimulus distributions but progressively evolve task-specific representations sensitive to distribution shifts.

\input{./figures-code/self-supervised}

% \paragraph{Alignment Over Training.}
% \textcolor{red}{Fig.~\ref{fig:self-supervised}-C shows how a Procrustes-based correlation score evolves between a pair of MoCo-trained networks across training. As in the supervised regime (Sec.~\ref{sec: convergence-dynamics}), the bulk of representational alignment appears in the first epoch---well before optimal task performance.}
% %In Fig.~\ref{fig:self-supervised}-C, we show how the correlation score computed using the Procrustes alignment metric for a pair of networks evolves over training. Consistent with our findings in the supervised regime (Sec.~\ref{sec: convergence-dynamics}), the bulk of representational alignment occurs in the first epoch---well before task performance has peaked.

% \paragraph{Sensitivity To Permutation Alignment.} 
% \textcolor{red}{Applying a random orthogonal rotation to the converged basis substantially drops permutation alignment (Fig.~\ref{fig:self-supervised})---consistent with supervised networks. This indicates that regardless of the learning paradigm, networks converge on a privileged coordinate basis.}
% %We apply a random rotation to the converged basis of MoCo-trained models. Consistent with our earlier findings, this perturbation leads to a significant drop in permutation alignment (Fig.~\ref{fig:self-supervised}-D). These results suggest that regardless of the learning paradigm, networks converge to a privileged basis.



==> yztwgkssnyyscymchgzppyswgzfcqwzw/vit.tex <==
\subsection{Representational Convergence in Vision Transformers}
\label{sec: vit-alignment}
%\textcolor{red}{We next analyze representational convergence in Vision Transformers (ViTs). All model and training details are in Appendix~\ref{sec: network-training}. For each layer, we use the [\texttt{CLS}] (class) token as a proxy for a layers representational geometry\footnote{Our underlying assumption here hinges on the fact that the [\texttt{CLS}] token aggregates the \emph{``information content''} of all patch embeddings via the self-attention operator. In addition, computing representational similarity for [\texttt{CLS}] vectors avoids having to deal with pooling patch similarities into a single representative score.}.}
We next analyze representational convergence in ViTs. All models and training details are in Appendix~\ref{sec: network-training}. We analyze the [\texttt{CLS}] (class) token representations at each layer. This is because the [\texttt{CLS}] token aggregates the \emph{``information content''} of all patch embeddings via the self-attention operator, making it a useful proxy to study representational geometry. In addition, computing representational similarity for [\texttt{CLS}] vectors avoids having to deal with pooling patch similarities into a single representative score.
\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.7\textwidth, keepaspectratio]{./figures/vit-alignment/vit.pdf}
    \caption{\textbf{Representational Convergence in Vision Transformers.} \textbf{(A)} We plot the evolution of alignment scores of three metrics (\textcolor{mplblue}{Linear}, \textcolor{mplorange}{Procrustes}, \textcolor{mplgreen}{Permutation}) computed between different seeds of the same ViT, which was trained on ImageNet. Error bars denote the standard deviation across $5$-fold cross validation. \textbf{(B)} We plot the inter-model orthogonal Procrustes (\textbf{left}) and permutation (\textbf{right}) scores for all layer pairs. Gray line plots denote the maximum alignment value over rows (right line) and columns (top line). \textbf{(C)} We visualize the evolution of the orthogonal Procrustes score at different checkpoints, ranging from epochs $0$ (untrained) to $25$. Darker colors correspond to epoch progression. \textbf{(D)} We rotate the converged basis of ViTs by a random rotation matrix and recompute the permutation scores for models trained ImageNet. Each dot represents a layer in the ViT. The permutation alignment remains approximately constant in both cases.}
    \label{fig:vit-alignment}
\end{figure}

\textbf{Results.} Analyses parallel to DCNNs reveal three key findings: 
(1) \textbf{Depth-wise convergence:} alignment tapers with network depth across metrics (Fig.~\ref{fig:vit-alignment}-A); \textcolor{mplorange}{Procrustes} and \textcolor{mplblue}{Linear} scores remain comparable, indicating rotations/reflections explain most inter-seed variability, and layer-wise patterns mirror DCNNs (Fig.~\ref{fig:vit-alignment}-B, left). 
(2) \textbf{No privileged axes:} independent ViT runs do not share a common basis—permutation scores between native and rotated axes are statistically indistinguishable across layers (Fig.~\ref{fig:vit-alignment}-D; Appendix~\ref{sec: basis-alignment-cnn-vit}). 
(3) \textbf{Early plateau:} alignment stabilizes after the first epoch, except for a \texttt{[CLS]} embedding artifact due to uniform positional encoding, indicating late-stage training does not drive convergence (Fig.~\ref{fig:vit-alignment}-C).


% \textbf{Results.} We conduct analyses akin to DCNNs, yielding several key insights on the following fronts:
% \begin{enumerate}
%     \item \textbf{Convergence Over Network Depth:} 
%     \textcolor{red}{Identical to DCNNs, alignment consistently tapers with network depth across all metrics (Fig.~\ref{fig:vit-alignment}-A). Moreover, linear and Procrustes scores remain comparable, indicating that inter-seed variability can largely be explained by rotations/reflections. Further, the layer-wise Procrustes score reveals an identical pattern to DCNNs (Fig.~\ref{fig:vit-alignment}-B, left).}
%     %Identical to DCNNs, we observe a consistent downward trend of alignment scores with network depth across all metrics in Fig.~\ref{fig:vit-alignment}-A. In addition, the Procrustes and linear alignments follow each other closely, again, suggesting that rotations and reflections can explain much of the variance in learned representations of ViTs. Further, the layer-wise alignment computed using the Procrustes metric reveals a pattern similar to DCNNs (Fig.~\ref{fig:vit-alignment}-B, left). 
%     \item \textbf{Absence of privileged axes in ViTs:} 
%     \textcolor{red}{Unlike DCNNs, independent ViT runs do not converge to a shared basis---permutation scores between native and rotated axes are statistically indistinguishable across layers (Fig.~\ref{fig:vit-alignment}-D). We discuss possible reasons for this difference in basis alignment in DCNNs vs. ViTs in Appendix~\ref{sec: basis-alignment-cnn-vit}.}
%     %Unlike DCNNs, independent runs of the same ViT architecture do not converge to similar bases, and permutation scores between native and rotated axes remain statistically indistinguishable across all layers. This indicates that ViTs do not develop consistent, shared axes of representation across training seeds (Fig.~\ref{fig:vit-alignment}-D). We provide a detailed explanation for basis alignment in DCNNs vs. ViTs in Appendix~\ref{sec: basis-alignment-cnn-vit}.
%     \item \textbf{Early plateau of alignment in ViTs:}
%     \textcolor{red}{Alignment largely stabilizes after the first epoch, except for an initialization  (uniform positional encoding) artifact in the \texttt{[CLS]} embedding. This implies that late-stage training does not drive convergence (Fig.~\ref{fig:vit-alignment}-C).}
%     %Consistent with DCNNs, alignment across different ViT seeds shows no systematic increase after epoch 1 for any layer except the input embedding, implying that late-stage training does not drive convergence (Fig.~\ref{fig:vit-alignment}-C). The [\texttt{CLS}] token’s apparent alignment spike at initialization is likely an artifact of its uniform positional encoding and weight initialization rather than true inter‐seed convergence.
% \end{enumerate}
